Chiral quantum heating and cooling with an optically controlled ion

Quantum heat engines and refrigerators are open quantum systems, whose dynamics can be well understood using a non-Hermitian formalism. A prominent feature of non-Hermiticity is the existence of exceptional points (EPs), which has no counterpart in closed quantum systems. It has been shown in classical systems that dynamical encirclement in the vicinity of an EP, whether the loop includes the EP or not, could lead to chiral mode conversion. Here, we show that this is valid also for quantum systems when dynamical encircling is performed in the vicinity of their Liouvillian EPs (LEPs) which include the effects of quantum jumps and associated noise - an important quantum feature not present in previous works. We demonstrate, using a Paul-trapped ultracold ion, the first chiral quantum heating and refrigeration by dynamically encircling a closed loop in the vicinity of an LEP. We witness the cycling direction to be associated with the chirality and heat release (absorption) of the quantum heat engine (quantum refrigerator). Our experiments have revealed that not only the adiabaticity-breakdown but also the Landau-Zener-St\"uckelberg process play an essential role during dynamic encircling, resulting in chiral thermodynamic cycles. Our observations contributes to further understanding of chiral and topological features in non-Hermitian systems and pave a way to exploring the relation between chirality and quantum thermodynamics.

==> ref.tex <==
\bibitem{science-352-235}  J. Ro$\beta$nagel, S. T. Dawkins, K. N. Tolazzi, O. Abah, E. Lutz, F. Schmidt-Kaler, \& K. Singer,
A single-atom heat engine,
{\it Science\/} \textbf{352}, 325 (2016).

\bibitem{PRL-123-080602} D. von. Lindenfels, O. Gr\"{a}b,  C. T. Schmiegelow,  V. Kaushal, J. Schulz, M. T. Mitchison, J. Goold, F. Schmidt-Kaler,\& U. G. Poschinger,
Spin Heat Engine Coupled to a Harmonic-Oscillator Flywheel,
{\it Phys. Rev. Lett.\/} {\bf 123}, 080602 (2019).

\bibitem{PRL-100-140501} C. A. Ryan, O. Moussa, J. Baugh, \& R. Laflamme,
Spin Based Heat Engine: Demonstration of Multiple Rounds of Algorithmic Cooling,
{\it Phys. Rev. Lett.\/} {\bf 100}, 140501 (2008).

\bibitem{PRL-123-240601} J. P. S. Peterson, T. B. Batalh$\tilde{a}$o, M. Herrera, A. M. Souza, R. S. Sarthour, I. S. Oliveira, \& R. M. Serra, Experimental Characterization of a Spin Quantum Heat Engine,
{\it Phys. Rev. Lett.\/} {\bf 123}, 240601 (2019).

\bibitem{PNAS-111-13786} J. V. Koski, V. F. Maisi, J. P. Pekola, \& D. V. Averin,
Experimental realization of a Szilard engine with a single electron,
{\it Proc. Natl. Acad. Sci. U.S.A.\/} {\bf 111}, 13786 (2014).

\bibitem{PRL-125-166802} K. Ono, S. N. Shevchenko, T. Mori, S. Moriyama, \& F. Nori,
Analog of a Quantum Heat Engine Using a Single-Spin Qubit,
{\it Phys. Rev. Lett.\/} {\bf 125}, 166802 (2020).

\bibitem{PRL-122-110601} J. Klatzow, J. N. Becker, P. M. Ledingham, C. Weinzetl, K. T. Kaczmarek,
D. J. Saunders, J. Nunn, I. A. Walmsley, R. Uzdin, \& E. Poem,
Experimental Demonstration of Quantum Effects in the Operation of Microscopic Heat Engines,
{\it Phys. Rev. Lett.\/} {\bf 122}, 110601 (2019).

\bibitem{PRL-97-180402} H. T. Quan, Y. D. Wang, Y. X. Liu, C. P. Sun, \& F. Nori,
Maxwell Demon Assisted Thermodynamic Cycle in Superconducting Quantum Circuits,
{\it Phys. Rev. Lett.\/} {\bf 97}, 180402 (2006).

\bibitem{PRL-112-150602} K. Zhang, F. Bariani, \& P. Meystre,
Quantum optomechanical heat engine,
{\it Phys. Rev. Lett.\/} {\bf 112}, 150602 (2014).

\bibitem{PRL-114-183602} A. Dechant, N. Kiesel, \& E. Lutz,
All-Optical Nanomechanical Heat Engine,
{\it Phys. Rev. Lett.\/} {\bf 114}, 183602 (2015).

\bibitem{ARPC-65-365} R. Kosloff, \& A. Levy,
Quantum Heat Engines and Refrigerators: Continuous Devices,
{\it Annu. Rev. Phys. Chem.\/} {\bf  65}, 365 (2014).

\bibitem{PRL-108-120602} A. Mari, \& J. Eisert,
Cooling by Heating: Very Hot Thermal Light Can Significantly Cool Quantum Systems,
{\it Phys. Rev. Lett.\/} {\bf 108}, 120602 (2012).

\bibitem{Eur-97-40003} A. Levy, \& R. Kosloff,
Quantum Absorption Refrigerator,
{\it Phys. Rev. Lett.\/} {\bf 108}, 070604 (2012).

\bibitem{PRB-94-235420} K. Y. Tan, M. Partanen,  R. E. Lake, J. Govenius, S. Masuda, \& M. M\"{o}tt\"{o}nen,
Quantum-circuit refrigerator.
{\it Nat. Commun.\/} {\bf 8}, 15189 (2017).

\bibitem{PRL-110-256801} D. Venturelli, R. Fazio, \& V. Giovannetti,
Minimal Self-Contained Quantum Refrigeration Machine Based on Four Quantum Dots,
{\it Phys. Rev. Lett.\/} {\bf 110}, 256801 (2013).

\bibitem{Natcommum-10-202} G. Maslennikov, S. Q. Ding, R. Hablutzel, J. Gan,
A. Roulet, S. Nimmrichter, J. Dai, V. Scarani, \& D. Matsukevich,
Quantum absorption refrigerator with trapped ions,
{\it Nat. Commun.\/} {\bf 10}, 202 (2019).

\bibitem{QST-1-015001} M. T. Mitchison, M. Huber, J. Prior, M. P. Woods, \& M. B. Plenio,
Realising a quantum absorption refrigerator with an atom-cavity system,
{\it Quantum Sci. Technol.\/} {\bf 1}, 015001 (2016).

\bibitem{science-363-42} M.-A. Miri, \& A. Al\`{u},
Exceptional points in optics and photonics,
{\it Science\/} {\bf 363}, 42 (2019).

\bibitem{Natmater-18-783} \c{S}. K. \"{O}zdemir, S. Rotter, F. Nori, \& L.Yang,
Parity-time symmetry and exceptional points in photonics,
{\it Nat. Mater.\/} \textbf{18}, 783 (2019).

\bibitem{science-364-878} Y. Wu, W. Liu, J. Geng, X. Song, X. Ye, C.-K. Duan, X. Rong, \& J. Du,
Observation of parity-time symmetry breaking in a single-spin system,
{\it Science\/} \textbf{364}, 878 (2019).

\bibitem{nature-607-271} Y. S. S. Patil, J. H{\"o}ller, P. A. Henry, C. Guria,
Y. Zhang, L. Jiang, N. Kralj, N. Read, \& J. G. E. Haris,
Measuring the knot of non-Hermitian degeneracies and non-commuting braids,
{\it Nature (London)\/} {\bf 607}, 271 (2022).

\bibitem{science-376-184} M. S. Ergoktas, S. Soleymani, N. Kakenov, K. Y. Wang, T. B. Smith, G. Bakan, S. Balci,
A. Principi, K. S. Novoselov,  \c{S}. K. {\"O}zdemir, C. Kocabas,
Topological engineering of terahertz light usingelectrically tunable exceptional point singularities,
{\it Science\/} \textbf{376}, 184(2022).

\bibitem{NC-13-599} S. Soleymani, Q. Zhong, M. Mokim, S. Rotter, R. E. Ganainy, \& \c{S}. K. \"{O}zdemir,
Chiral and degenerate perfect absorption on exceptional surfaces,
{\it Nat. Commun.} {\bf 13}, 599 (2022).

\bibitem{NP-15-1232} M. Naghiloo, M. Abbasi, Y. N. Joglekar, \&  K. W. Murch,
Quantum state tomography across the exceptional point in a single dissipative qubit,
{\it Nat. Phys.} {\bf 15}, 1232 (2019).

\bibitem{prl-126-083604} L. Y. Ding, K. Y. Shi, Q. X. Zhang, D. N. Shen, X. Zhang, \& W. Zhang,
Experimental Determination of $\mathcal{PT}$-Symmetric Exceptional Points in a Single Trapped Ion,
{\it Phys. Rev. Lett.\/} {\bf 126}, 083604 (2021).

\bibitem{prl-128-160401} M. Abbasi, W. J. Chen, M. Naghiloo, Y. N. Joglekar,\& K. W. Murch,
Topological Quantum State Control through Exceptional-Point Proximity,
{\it Phys. Rev. Lett.\/} {\bf 128}, 160401 (2022).

\bibitem{LEP} F. Minganti, A. Miranowicz, R. W. Chhajlany, \& F. Nori,
Quantum exceptional points of non-Hermitian Hamiltonians and Liouvillians: The effects of quantum jumps,
{\it Phys. Rev. A\/} {\bf 100}, 062131 (2019).

\bibitem{PRX-Quantum-2-040346} S. Khandelwal, N. Brunner, \& G. Haack,
Signatures of Liouvillian Exceptional Points in a Quantum Thermal Machine,
{\it Phys. Rev. X. Quantum.\/} {\bf 2}, 040346 (2021).

\bibitem{arXiv:2111.04754} W. J. Chen, M. Abbasi, B. Ha, S. Erdamar, Y. N. Joglekar, \& K. W. Murch,
Decoherence Induced Exceptional Points in a Dissipative Superconducting Qubit,
{\it Phys. Rev. Lett.\/} {\bf 128}, 110402 (2022).

\bibitem{PRL-126-170506} W. Liu, Y. Wu, C.-K. Duan, X. Rong,\& J. Du,
Dynamically Encircling an Exceptional Point in a Real Quantum System,
{\it Phys. Rev. Lett.\/} {\bf 126}, 170506 (2021).

\bibitem{nature-537-76} J. Doppler, A. A. Mailybaev, P. Rabl, N. Moiseyev, \& S. Rotter,
Dynamically encircling an exceptional point for asymmetric mode conversion,
{\it Nature (London)\/} {\bf 537}, 76 (2016).

\bibitem{prx-8-021066} X.-L. Zhang, S. Wang, B. Hou, \& C. T. Chan,
Dynamically Encircling Exceptional Points: In situ Control of Encircling Loops and the Role of the Starting Point,
{\it Phys. Rev. X \/} {\bf 8}, 021066 (2018).

\bibitem{prl-124-153903} Q. Liu, S. Li, B. Wang, S., Ke, C. Qin, K. Wang, W. Liu, D. Gao, P. Berini, \& P. Lu,
Efficient Mode Transfer on a Compact Silicon Chip by Encircling Moving Exceptional Points,
{\it Phys. Rev. Lett.\/} {\bf 124}, 153903 (2020).

\bibitem{prl-125-187403} A. Li, J. Dong, J. Wang, Z. Cheng, J. S. Ho,
D. Zhang, J. Wen, X.-L. Zhang, C. T. Chan, A. Al\'{u}, C.-W. Qiu, \& L. Chen,
Hamiltonian Hopping for Efficient Chiral Mode Switching in Encircling Exceptional Points,
{\it Phys. Rev. Lett.\/} {\bf 125}, 187403 (2020).

\bibitem{nature-562-86} J. W. Yoon, Y. Choi, C. Hahn, G. Kim, S. H. Song, K.-Y. Yang,
J. Y. Lee, Y. Kim, C. S. Lee, J. K. Shin, H.-S. Lee, \&  P.Berini,
Time-asymmetric loop around an exceptional point over the full optical communications band,
{\it Nature (London)\/} {\bf 562}, 86 (2018).


\bibitem{pra-96-052129} A. U. Hassan, G. L. Galmiche, G. Harari, P. LiKamWa, M. Khajavikhan, M.  Segev,\& D. N. Christodoulides,
Chiral state conversion without encircling an exceptional point,
{\it Phys. Rev. A\/} {\bf 96}, 052129 (2017).

\bibitem{Natcommum-9-4808} Q. Zhong, M. Khajavikhan, D. N. Christodoulides, \& R. El-Ganainy,
Winding around non-Hermitian singularities,
{\it Nat. Commun.\/} {\bf 9}, 4808 (2018).

\bibitem{pra-102-040201} J. Feilhauer, J. Doppler, A. A. Mailybaev, J. B{\"o}hm, U.  Kuhl, N.  Moiseyev,\& S. Rotter,
Encircling exceptional points as a non-Hermitian extension of rapid adiabatic passage,
{\it Phys. Rev. A\/} {\bf 102}, 040201 (2020).

\bibitem{nature-605-256} H. Nasari, G. Lopez-Galmiche, H. E. Lopez-Aviles, A. Schumer,
A. U. Hassan, Q. Zhong, S. Rotter, P. LikamWa,  D. N. Christodoulides, \& M. Khajavikhan,
Observation of chiral state transfer without encircling an exceptional point,
{\it Nature \/} {\bf 605}, 256 (2018).

\bibitem{nature-537-80} H. Xu, D. Mason, L. Y. Jiang, \& J. G. E. Harris,
Topological energy transfer in an optomechanical system with exceptional points,
{\it Nature (London)\/} {\bf 537}, 80 (2016).

\bibitem{LZS} S. N. Shevchenko, S.  Ashhab \& F. Nori,
Landau-Zener-St{\"u}ckelberg interferometry,
{\it Phys. Rep.} {\bf 492}, 1 (2010).

\bibitem{SA-2-e1600578} F. Zhou, L. L. Yan, S. J. Gong, Z. H. Ma, J. Z. He, T. P. Xiong, L. Chen, W. L. Yang, M. Feng, \& V. Vedral,
Verifying Heisenberg's error-disturbance relation using a single trapped ion,
{\it Sci. Adv.} {\bf 2}, e1600578 (2016).

\bibitem{njp-19-063032} T. P. Xiong, L. L. Yan, F. Zhou, K. Rehan, D. F. Liang, L. Chen, W. L. Yang, Z. H. Ma, M. Feng, \& V. Vedral,
Experimental verification of a Jarzynski-related information-theoretic equality using a single trapped ion,
{\it Phys. Rev. Lett.} {\bf 120}, 010601 (2018).


\bibitem{PRR-2-033082} J. W. Zhang, K. Rehan, M. Li, J. C. Li, L. Chen, S. L. Su, L. L. Yan, F. Zhou, \& M. Feng,
Single-atom verification of the information-theoretical bound of irreversibility at the quantum level,
{\it Phys. Rev. Research} {\bf 2}, 033082 (2020).

\bibitem{NC-2022} J.-W. Zhang, J.-Q. Zhang, G.-Y. Ding, J.-C. Li, J.-T. Bu, B. Wang,
L.-L. Yan, S.-L. Su, L. Chen, F. Nori,  \c{S}. K. \"{O}zdemir, F. Zhou, H. Jing, \& M. Feng,
Dynamical Control of Quantum Heat Engines Using Exceptional Points,
{\it Nat. Commun.} {\bf 13}, 6225 (2022).

\bibitem{explain1} In this model, we can engineer both the Rabi frequency $\Omega$ and the effective dacay rate $\gamma_{\mathrm{eff}}=\tilde{\Omega}^{2}/\Gamma$ under the condition of $\Omega\ll\tilde{\Omega}$ \cite{PRR-2-033082, NC-2022}. With this level of controllability, we can fully tune this two-level system and perform parametric loops that encircle or do not encircle the LEP.

\bibitem{SM} See Supplementary Materials.

\bibitem{huber} J. Huber, P. Kirton, S. Rotter, \& P. Rabl,
Emergence of $\mathcal{PT}$-symmetry breaking in open quantum systems,
{\it Sci-Post Phys.\/} {\bf 9}, 52 (2020).

\bibitem{naka} Y. Nakanishi, \& T. Sasamoto,
PT phase transition in open quantum systems with Lindblad dynamics,
{\it Phys. Rev. A} {\bf 105}, 022219 (2020).

\bibitem{LZtransition} L. Landau,
On the theory of transfer of energy at collisions II,
{\it Phys. Z. Sowjetunion} {\bf 2}, 46 (1932);
C. Zener,
Non-Adiabatic Crossing of Energy Levels,
Proc. R. Soc. Lond. A {\bf 137}, 696 (1932).

\bibitem{Sphase} E. C. G. St{\"u}ckelberg,
Theory of inelastic collisions between atoms,
{\it Helv. Phys. Acta} {\bf 5}, 369 (1932).

\bibitem{prl-118-033901} Q. T. Cao, H. Wang, C. H. Dong, H. Jing, R. S. Liu, X. Chen, L. Ge, Q. Gong, and Y. F. Xiao, 
Experimental Demonstration of Spontaneous Chirality in a Nonlinear Microresonator, 
{\it Phys. Rev. Lett.} {\bf 118}, 033901 (2017).

\bibitem{lsa-8-88} X. L. Zhang, T. Jiang, and C. T. Chan, 
Dynamically encircling an exceptional point in anti-parity-time symmetric systems: asymmetric mode switching for symmetry-broken modes, 
{\it Light Sci. Appl.} {\bf 8}, 88 (2019).

\bibitem{lsa-12-87} S. Baek, S. H. Park, D. Oh, K. Lee, S. Lee, H. Lim, T. Ha, H. S. Park, S. Zhang, L. Yang, B. Min, and T. T. Kim, 
Non-Hermitian chiral degeneracy of gated graphene metasurfaces, 
{\it Light Sci. Appl.} {\bf 12}, 87 (2023).
